Multiplicity dependence of $\pi$, K, and p production in pp collisions at $\sqrt{s} = 13$ TeV

This paper presents the measurements of $\pi^{\pm}$, $\rm{K}^{\pm}$, $\rm{p}$ and $\bar{\rm{p}}$ transverse momentum ($p_{\rm{T}}$) spectra as a function of charged-particle multiplicity density in proton-proton (pp) collisions at $\sqrt{s}$ = 13 TeV with the ALICE detector at the LHC. Such study allows us to isolate the center-of-mass energy dependence of light-flavour particle production. The measurements reported here cover a $p_{\rm{T}}$ range from 0.1 GeV/$c$ to 20 GeV/$c$ and are done in the rapidity interval $|y|<0.5$. The $p_{\rm{T}}$-differential particle ratios exhibit an evolution with multiplicity, similar to that observed in pp collisions at $\sqrt{s}$ = 7 TeV, which is qualitatively described by some of the hydrodynamical and pQCD-inspired models discussed in this paper. Furthermore, the $p_{\rm{T}}$-integrated hadron-to-pion yield ratios measured in pp collisions at two different center-of-mass energies are consistent when compared at similar multiplicities. This also extends to strange and multistrange hadrons, suggesting that, at LHC energies, particle hadrochemistry scales with particle multiplicity the same way under different collision energies and colliding systems.

==> Data_Analyses/CorrAndNorm.tex <==
The raw particle distributions are normalized to the total number of events analysed\footnote{Events that passed all the selection criteria.} in each multiplicity class. To obtain the \pT distributions of primary \pion, \kaon, and \pr, the raw particle distributions obtained from the different PID approaches need to be also corrected for the detector efficiency and acceptance, the ITS-TPC, and TPC-TOF matching efficiency, the PID efficiency, the trigger efficiency and the contamination from secondary particles.\\
Secondary particles are either produced in weak decays or from the interaction of particles with the detector material.
The estimation of secondary particle contribution is based on the Monte Carlo (MC) templates of the distance of closest approach of the track to the primary vertex in the transverse plane with respect to the beam axis (DCA$_{xy}$), as carried out in previous works~\cite{Abelev:2013vea, Acharya:2018orn}. The DCA$_{xy}$ distributions of the tracks in data are fitted with three MC templates corresponding to the expected shapes of primary particles, secondaries from material and secondaries from weak decays to obtain the correct fraction of primary particles in the data. This procedure is repeated in each \pT and multiplicity bin and thus takes into account the possible differences in the feed-down corrections due to the change in the abundances and spectral shapes of the weakly decaying particles. The contamination is different in each PID analysis due to different track selection criteria and PID techniques and hence it is estimated separately for each analysis. The contribution of secondary particles was found to be significant for \pion (up to 2\%) and \pr (up to 15\%) whereas the contribution for \kaon is negligible. \\
The spectra are corrected for the detector acceptance and track reconstruction efficiencies based on a simulation using the \pythiaeight (Monash-2013 tune) Monte Carlo event generator \cite{Skands:2014pea} and particle propagation through the full ALICE geometry using GEANT3~\cite{Brun:1119728}. In this simulation, tracks are reconstructed using the same algorithms as for the data. The detector acceptance and reconstruction efficiencies are found to be independent of charged-particle multiplicity and thus the multiplicity-integrated values are used in all multiplicity classes.
As GEANT3 does not fully describe the interaction of low-momentum \pbar and \kam with the detector material, an additional correction factor to the efficiency for these two particles is estimated with GEANT4~\cite{Agostinelli:2002hh} and FLUKA~\cite{Ferrari:2005zk}, respectively, where the interaction processes are known to be better reproduced \cite{Abelev:2013vea}. Additional corrections to the efficiency are applied when TPC or TOF information is used to take into account the track matching between ITS and TPC, and between TPC and TOF.
\\
%Concerning the particle distributions obtained with the TPC and TOF detectors, an additional correction to the efficiency takes into account the matching of TPC tracks with ITS hits and the matching of TPC tracks to TOF (in the TOF \pT range). \\
Signal losses due to the trigger selection are extracted from \pythiaeight (Monash-2013 tune) MC simulation as performed in~\cite{Acharya:2019kyh}.
The correction is found to be 17--18\% at low \pT in the V0M class X (the lowest multiplicity), and reduces to $\sim$5\%, $\sim$2\% in classes IX and VIII, respectively. The correction is negligible in higher multiplicity pp collisions and for \pT $\gtrsim$ 4 GeV/$c$ in all multiplicity bins except in class X. In the latter, the correction reaches $\sim$2\% at \pT = 7 GeV/$c$. %The correction shows a small dependence with the particle species within $1\%$. A systematic uncertainty is applied to consider dependencies on the event generator.\\
%\footnote{The true inelastic events are those with at least one primary charged particle in $|\eta^{\rm true}|$ $<$ 1 and with the primary vertex in the region $|V^{\rm true}_{\rm z}|$ $<$ 10 cm.}
Finally, an additional correction is applied to pass from triggered INEL$>$0 to true INEL$>0$ events, i.e. events with at least one primary charged particle in $|\eta^{\rm true}|$ $<$ 1 and with the primary vertex in the region $|V^{\rm true}_{\rm z}|$ $<$ 10 cm. The correction is independent of particle species and is found to be negligible from V0M I (the highest multiplicity) to V0M VI, while it ranges from 1\% in class VII to 11\% in class X. The correction is about 8\% for multiplicity-integrated INEL$>0$ events.


==> Data_Analyses/Systematics.tex <==
The systematic uncertainties are divided into two categories, those common to all analyses and those which are analysis specific.
The common systematic uncertainties are those due to tracking, which includes track quality criteria and the \pt-dependent ITS-TPC matching efficiency (except for the ITSsa analysis), the TPC-TOF matching efficiency (for TPC-TOF and TOF analyses), and the signal loss correction. In addition, the systematic source related to the effect of the material budget on the global tracking (\pT dependent) is also added. The uncertainties on global tracking and TPC-TOF matching due to material budget are calculated by varying the material budget in the simulation by $\pm$ 5\%. The uncertainty related to the hadronic interaction cross section in the detector material is estimated using GEANT4~\cite{Agostinelli:2002hh} and FLUKA~\cite{Ferrari:2005zk} transport codes. Finally, an additional systematic uncertainty of 2\% is added to account for possible multiplicity dependence of track reconstruction efficiency and signal loss correction calculated from a MC simulation.
All common sources of systematic uncertainties are summarised in \tab{syspikp}.
In the same table, the individual analysis systematic uncertainties are also listed for each particle species.

The estimation of the systematic uncertainties for the ITSsa analysis is described in detail in \cite{Abelev:2013vea, Acharya:2018orn}.
The ITSsa tracking uncertainties are estimated by varying the main criteria for the track selection, namely those on the DCA$_{xy}$, on the $\chi^{2}$ of the track, and on the number of clusters required in the ITS layers.
The uncertainty related to the particle identification is calculated by using a Bayesian technique and comparing the results obtained with the standard n$\sigma$ method as already performed in \cite{Adam:2016dau}.
Due to the Lorentz force, the positions of ITS clusters are shifted depending on the magnetic field polarity, giving rise to a 3\% uncertainty.
Finally, the energy-independent uncertainty related to the ITS material budget is estimated with a simulation of pp collisions at $\sqrt{\rm s}$ = 900 GeV by varying the material budget of the ITS by $\pm$7.5\%  \cite{Aamodt:2011zj}.
For the TPC-TOF fits analysis at low \pT (below 500, 600, and 800 \MeVc for \pion, \kaon, and \pr, respectively), the systematic uncertainty associated with the PID technique is calculated by integrating the measured $\textrm{d}E/\textrm{d}x$ of charged tracks in the ranges of $\pm3.5\sigma$ and $\pm2.5\sigma$, where $\sigma$ represents one standard deviation from the $\langle\textrm{d}E/\textrm{d}x\rangle$ under given mass hypothesis.
At higher \pT values, where only the time-of-flight information is used, the associated uncertainties are calculated by simultaneously varying the width and tail parameters by 10\%. An additional uncertainty is calculated by fixing the central values of the fit functions to the $\beta$ calculated for each particle species in a given momentum range. This was found to be the dominant source of systematic uncertainty for \pion and \kaon at the highest \pT values ($\gtrsim 2.5~\GeVc$).
For the TOF template fits analysis, PID uncertainties are estimated by simultaneously varying the spread and tail slope of each $\Delta t$ template by 10\%. In addition to this, for both the TPC-TOF and TOF template fits analyses, systematic uncertainties associated with tracking are calculated by varying the track selection criteria: the number of crossed rows in the TPC, the distance of closest approach in beam and transverse directions, and the quality of the global track fit $\chi^{2}$.
For the kink analysis the sources of systematic uncertainties are: the kink vertex finding efficiency (3\% constant in \pt), the kink PID efficiency (calculated by taking into account the position of the kink vertex), the number of TPC clusters of the decaying particle track and the $q_{\rm T}$ of the decay product, and the uncertainty related to the purity of the selected sample.
The contamination due to the random association of tracks wrongly attributed to kaon decays is of the order of 2.3\% at low transverse momenta and reaches the value of 3.4\% above 4 GeV/$c$.
The largest component of the systematic uncertainties in the analysis of the relativistic rise of the TPC arises from the imprecise parametrization of both the Bethe-Bloch and resolution curves.
%The technique adopted to estimate the systematic uncertainties in the spectra is described in~\cite{Adam:2015kca}.
To quantify this uncertainty, the variations of the Bethe-Bloch resolution parametrizations with respect to the measured $\langle {\rm d}E/{\rm d}x \rangle(\sigma_{\langle {\rm d}E/{\rm d}x \rangle})$ are used to vary the values of the mean and $\sigma$ in the 4-Gaussian fit~\cite{Adam:2015kca}.
The largest relative deviation between the nominal particle ratios and the ones obtained after the variations are assigned as a systematic uncertainty.












\input{Inputs/Tables/SpectraSystTable.tex}


==> Tables/PIDpTRanges.tex <==
\begin{table*}[!h]
%\centering
\label{PIDpt}
  \caption{Different \pt ranges used for the identification of pions, kaons and protons. The final \pt spectra have been obtained by combining the results of the various PID techniques.}
  \label{tab:PIDptpikp}
  \begin{tabularx}{\textwidth}{p{3.0cm}*{2}{Y}*{2}{Y}*{2}{Y}*{4}{Y}}
\hline\hline

 \multirow{2}{*}{Analysis} & \multirow{2}{*}{PID Technique} & \multicolumn{6}{c}{\pt ranges (\GeVc)} & (pseudo)rapidity\\
    &  & \multicolumn{2}{c}{\pipm} & \multicolumn{2}{c}{\kapm} & \multicolumn{2}{c}{\p\ (\pbar)} & range \\
    \hline \\

	ITSsa & n$\sigma$ integral  & \multicolumn{2}{c}{0.1$-$0.7} & \multicolumn{2}{c}{0.2$-$0.6} & \multicolumn{2}{c}{0.3$-$0.65} & $|y|<$0.5 \\ \\

	TPC-TOF fits & \specialcell{n$\sigma$ fits to TPC,\\ $\beta$ fits to TOF} & \multicolumn{2}{c}{0.25$-$3.0} & \multicolumn{2}{c}{0.3$-$3.0} & \multicolumn{2}{c}{0.45$-$3.0} & \specialcell{$|y|<$0.5 (TPC)\\ $|\eta|<$0.4 (TOF)} \\ \\


	TOF template fits & \specialcell{Statistical\\ unfolding of $\Delta t$} & \multicolumn{2}{c}{0.7$-$4.0} & \multicolumn{2}{c}{0.6$-$3.0} & \multicolumn{2}{c}{0.9$-$4.0} & $|y|<$0.5 \\ \\


	Kinks & Kink topology & \multicolumn{2}{c}{$-$} & \multicolumn{2}{c}{0.35$-$6.0} & \multicolumn{2}{c}{$-$} & $|y|<$0.5 \\ \\

	rTPC & TPC d\textit{E}/d\textit{x} fits & \multicolumn{2}{c}{2$-$20} & \multicolumn{2}{c}{3$-$20} &  \multicolumn{2}{c}{3$-$20} & $|\eta|<$0.8 \\ \\



\hline \hline
	\end{tabularx}

%  ~\newline
\end{table*}


==> Tables/SpectraSystTable.tex <==
\begin{table*}[ph!]\label{syst}
\caption{Sources of the relative systematic uncertainties of the \pt-differential yields of \pion, \kaon,\ and \pr. The uncertainties are split into two categories, the common and the individual-analysis specific for low, intermediate and high \pt. Numbers in parenthesis in the \pr column refer to \pbar uncertainties. In the last rows, the maximum (among multiplicity classes) total systematic uncertainty is reported.}
\label{tab:syspikp}
  \begin{tabularx}{\textwidth}{p{5.3cm}*{2}{Y}*{1}{Y | }*{2}{Y}*{1}{Y | }*{3}{Y}}
\hline\hline
    &  \multicolumn{9}{c}{Uncertainty (\%)} \\
    {\bf Common source}  & \multicolumn{3}{c}{\pion} & \multicolumn{3}{c}{\kaon} & \multicolumn{3}{c}{\pr (\pbar)} \\
\hline
    \pt\ (\GeVc)   &   0.1 & 3.0 & 20.0   &   0.2 & 2.5 & 20.0 &   0.3 & 4.0 & 20.0   \\
    \hline
    %\cmidrule(l{5pt}){1-10}
    %\cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
%%% Common Uncertainties
% Not obvious: would we prefer quoting only 2 and not 3 pt ranges here?
% --- it might depend on the pT dendence of these systematics
    Correction for secondaries & 1  & 1 & \multicolumn{1}{c | }{1} & \multicolumn{3}{c | }{negl.} & 4 & 1 & 1 \\
    Hadronic interactions & 2 & 2.4 & 2.4 & 2.7 & 1.8 & 1.8 & 1\ (3.6) & 1\ (3.6) & 1\ (3.6) \\
    ITS-TPC matching efficiency  & 0.7 & 1.5 & 2.9 & 0.7 & 1.5 & 2.9 & 0.7 & 1.5 & 2.9\\
   Global tracking efficiency & \multicolumn{3}{c | }{0.7} & \multicolumn{3}{c | }{0.5} & \multicolumn{3}{c}{1.5} \\
   TOF matching efficiency \newline (TPC-TOF fits,TOF template fits) & \multicolumn{3}{c | }{\multirow{2}{*}{3}} & \multicolumn{3}{c | }{\multirow{2}{*}{6}} & \multicolumn{3}{c}{\multirow{2}{*}{4}} \\
   Signal-loss correction & \multicolumn{3}{c | }{0.2} & \multicolumn{3}{c | }{1} & \multicolumn{3}{c}{3.3} \\
   \hline
    \pt\ (\GeVc)   &   0.3 & 3.0 & 20.0   &   0.3 & 2.5 & 20.0 &   0.4 & 4.0 & 20.0   \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%	\cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
	Material budget \newline (TPC-TOF) & \multirow{2}{*}{0.5} & \multirow{2}{*}{1.0} & \multirow{2}{*}{0.2} & \multirow{2}{*}{1.5} & \multirow{2}{*}{1.0} & \multirow{2}{*}{0.4} & \multirow{2}{*}{2.9} & \multirow{2}{*}{1.7} & \multirow{2}{*}{0.1} \\
\hline
    {\bf Specific source} & \multicolumn{3}{c}{\pion} & \multicolumn{3}{c}{\kaon} & \multicolumn{3}{c}{\pr (\pbar)} \\
\hline
%%% ITS Standalone Analysis Uncertainties
    {\bf ITSsa}, \pt\ (\GeVc)   &   0.10 & & 0.70   &   0.20 & & 0.60 &   0.30 & & 0.65   \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
%    {\bf ITSsa}& \multicolumn{9}{c}{} \\
    Tracking & 1.4 &  & 1.4 & 1.5 &  & 1.5 & 1.1 &  & 1.1  \\
    Material budget & 4.8 & & 0.3 & 2.3 & & 0.6 & 5.0 & & 0.9 \\
    $E \times B$ effect & & 3.0 & & & 3.0 & & & 3.0 & \\
    PID & 0.4 & & 0.4 & 3.9 & & 3.9 & 4.2 & & 4.2 \\
\hline\hline

    %\pt\ (\GeVc)   &   0.2 &  & 2.5   &   0.3 & & 2.5  &   0.5 & & 2.5    \\
    %\cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    %Bayesian PID  & \multicolumn{3}{c}{1} & 1 & & 3 & 1 & & 2 \\   %\multicolumn{3}{c}{1.5\%} & \multicolumn{3}{c}{3.5\%} & \multicolumn{3}{c}{2.5\%} \\
%\hline\hline

    {\bf TOF templates}, \pt\ (\GeVc)   &   0.7 &  & 4.0   &   0.6 & & 3.0  &   0.9 & & 4.0    \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    PID & 1 & & 9.4 & 1 & & 12 & 1 & & 21  \\
    %TPC-TOF PID & \multicolumn{3}{c}{1} & 1 & & 5 & \multicolumn{3}{c}{1} \\
\hline\hline

    {\bf TPC-TOF fits}, \pt\ (\GeVc)   &   0.3 &  & 3   &   0.3 & & 3  &   0.4 & & 3    \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    PID & 1.4 & & 7 & 3 & & 16 & 1 & & 4.3 \\
\hline\hline

    {\bf rTPC}, \pt\ (\GeVc)   &  2.0 &  & 20.0   &   2.0 & & 20.0  &   2.0 & & 20.0    \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    Bethe--Bloch parameterization & 8.1 &  & 4 & 14.8 &  & 8.0  & 14 & & 6.0 \\
    Feed-Down  & 0.5 &  & 0.5 & - &  & -  & 2.4 & & 2.0 \\
\hline\hline

    {\bf Kinks}, \pt\ (\GeVc)   &  0.6 &  & 6.0   &   0.6 & & 6.0  &   0.6 & & 6.0    \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    PID & - & & - & 0.75 & & 5.3  & - & & - \\
    Kink vertex finding efficiency & - & & - & 3 & & 3  & - & & - \\
    Contamination & - & & - & 2.3 & & 3.4  & - & & - \\
\hline\hline

   {\bf Total}  & \multicolumn{3}{c}{\pion} & \multicolumn{3}{c}{\kaon} & \multicolumn{3}{c}{\pr (\pbar)} \\
\hline
    \pt\ (\GeVc)   &   0.3 & 3.0 & 20.0   &   0.3 & 3.0 & 20.0 &   0.3 & 3.0 & 20.0   \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    Total & 6.6 & 5.1 & 4.3 & 6.6 & 6.8 & 7.8 & 9.6 & 9.7 & 12.4 \\
    \hline\hline

       {\bf Particle ratios}  & \multicolumn{3}{c}{K/$\pi$} & \multicolumn{3}{c}{p/$\pi$}  \\
\hline
    \pt\ (\GeVc)   &   0.2 & 3.0 & 20.0   &   0.3 & 3.0 & 20.0    \\
    \hline
%    \cmidrule(l{5pt}){1-10}
%    \cmidrule(l{5pt}){2-4} \cmidrule(l{5pt}){5-7} \cmidrule(l{5pt}){8-10}
    Total & 7.2 & 14.6 & 7.7 & 10.2 & 12.2 & 11.5 \\
   %  \hline\hline
 %   Total ($N_{ch}$-independent) & 8.1 & 4.4 & 6.9 & 6.7 & 6.1 & 12.2 & 10.5 & 13.5 & 11.5\\
    \bottomrule
  \end{tabularx}
  ~\newline
\end{table*}


==> Tables/mdNdeVsMulti.tex <==
\begin{comment}
\begin{table*}[ph!]
  \begin{center}
  \caption{Mean charged-particle multiplicity density \mdNde measured in different event multiplicity classes.}
  \label{tab:mdNdeTable}
%  \begin{tabularx}{\textwidth}{p{2 cm} X X X X X}
  \begin{tabular}{c c c c c c c c c c c}
    \hline \hline
    V0M mult. class & I & II & III & IV & V \\
    Frac. of INEL$>$0 (\%) & 0-1 & 1-5 & 5-10 & 10-15 & 15-20  \\
    \mdNde  & $26.02\pm0.35$ & $20.02\pm0.27$ & $16.17\pm0.22$ & $13.77\pm0.19$ & $12.04\pm0.17$  \\ \midrule
    V0M mult. class & VI & VII & VIII & IX & X\\
    Frac. of INEL$>$0 (\%) & 20-30 & 30-40 & 40-50 & 50-70 & 70-100 \\
    \mdNde  & $10.02\pm0.14$ & $7.95\pm0.11$ & $6.32\pm0.09$ & $4.50\pm0.07$ & $2.55\pm0.04$ \\  \bottomrule
  \end{tabular}
  \end{center}
\end{table*}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%% Updated table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!h]
  \begin{center}
%  \begin{tabularx}{\textwidth}{p{2 cm} X X X X X}
\caption{Mean charged-particle multiplicity density \mdNde measured in different event multiplicity classes. Multiplicity classes are selected based on the visible inelastic scattering cross-section. The fraction of the total inelastic scattering cross-section is quoted for each class in the central rows.}
\label{tab:mdNdeTable}
  \begin{tabular}{c c c c c c c c c c c}
    \hline \hline
    V0M mult. class & I & II & III & IV & V \\
    $\sigma$/$\sigma_{\rm INEL>0}$ (\%) & 0--0.92 & 0.92--4.6 & 4.6--9.2 & 9.2--13.8 & 13.8--18.4  \\
    \mdNde  & $26.02\pm0.35$ & $20.02\pm0.27$ & $16.17\pm0.22$ & $13.77\pm0.19$ & $12.04\pm0.17$  \\ \midrule
    V0M mult. class & VI & VII & VIII & IX & X\\
    $\sigma$/$\sigma_{\rm INEL>0}$ (\%) & 18.4--27.6 & 27.6--36.8 & 36.8--46.0 & 46.0--64.5 & 64.5--100 \\
    \mdNde  & $10.02\pm0.14$ & $7.95\pm0.11$ & $6.32\pm0.09$ & $4.50\pm0.07$ & $2.55\pm0.04$ \\  \bottomrule
  \end{tabular}
  \end{center}
\end{table*}

